GBT/MUSTANG-2 9" resolution imaging of the SZ effect in MS0735.6+7421: Confirmation of the SZ Cavities through direct imaging

Mechanical feedback from active galactic nuclei (AGN) is thought to be the dominant feedback mechanism quenching cooling flows and star formation in galaxy cluster cores. However, the mechanisms by which AGN couple to the intracluster medium (ICM) are not well understood. The nature of pressure supporting the cavities is not known. Using the MUSTANG-2 instrument on the Green Bank Telescope (GBT), we aimed to measure thermal Sunyaev-Zeldovich (SZ) effect signals associated with the X-ray cavities in MS0735.6+7421, a moderate mass cluster hosting one of the most energetic AGN outbursts known. We use these measurements to infer the level of non-thermal sources of pressure, such as magnetic fields and turbulence, as well as relativistic and cosmic ray components, supporting the cavities. We used preconditioned gradient descent to fit a model for the cluster, cavities, and central point source directly to the time ordered data of the MUSTANG-2 signal. We use this model to probe the thermodynamic state of the cavities. We have shown that the SZ signal associated with the cavities is suppressed compared to the expectations for a thermal plasma with the temperature $\sim$few tens keV. The smallest value of the suppression factor $f$ that is consistent with the data is $\sim$0.4, lower than inferred in earlier work. Larger values of $f$ are possible once the contribution of the cocoon shock surrounding the bubbles is taken into account. The baseline model with this particular geometrical setup yields best-fitting value f~0.5, which at face value implies a mix of thermal and non-thermal pressure support. Larger values of $f$ (up to 1, i.e. no tSZ signal from the bubbles) are still possible when allowing for variations in the line-of-sight geometry.

==> authors.tex <==
\author{John Orlowski-Scherer}\inst{1}%[0000-0003-1842-8104]
%\institute{E-mail: \href{mailto:jackorlowskischerer@gmail.com }{jackorlowskischerer@gmail.com } }
\institute{Department of Physics and Astronomy, University of Pennsylvania, 209 South 33rd Street, Philadelphia, PA, 19104, USA\\
              \email{jorlo@sas.upenn.edu}
              }
%\and
%\author{Saianeesh Keshav Haridas}%[0000-0001-6519-502X]
%\institute{Department of Physics and Astronomy, University of Pennsylvania, 209 South 33rd Street, Philadelphia, PA, 19104, USA}
%\and
%\author{Luca Di Mascolo}%[0000-0003-3586-4485]
%\institute{Department of Physics, University of Trieste, via Tiepolo 11, 34131 Trieste, Italy}
%\institute{INAF - Osservatorio Astronomico di Trieste, via Tiepolo 11, 34131 Trieste, Italy}
%\institute{IFPU - Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy}
%\and
%\author{Karen Perez Sarmiento}
%\institute{Department of Physics and Astronomy, University of Pennsylvania, 209 South 33rd Street, Philadelphia, PA, 19104, USA}
%\and
%\author{Charles E. Romero}%[0000-0001-5725-0359]
%\institute{Smithsonian Astrophysical Observatory, 60 Garden Street, Cambridge, MA 02143, USA}
%\and
%\author{Simon Dicker}%[0000-0002-1940-4289]
%\institute{Department of Physics and Astronomy, University of Pennsylvania, 209 South 33rd Street, Philadelphia, PA, 19104, USA}
%\and
%\author{Tanay Bhandarkar}%[0000-0002-2971-1776]
%\institute{Department of Physics and Astronomy, University of Pennsylvania, 209 South 33rd Street, Philadelphia, PA, 19104, USA}
%\and
%\author{Mark Devlin}
%\institute{Department of Physics and Astronomy, University of Pennsylvania, 209 South 33rd Street, Philadelphia, PA, 19104, USA}
%\and
%\author{Ian Lowe}
%\institute{Department of Astronomy, University of Arizona, Tucson, AZ 85721.}
%\and
%\author{Brian Mason}%[0000-0002-8472-836X]
%\institute{NRAO, 520 Edgemont Rd, Charlottesville, VA 22903}
%\and
%\author{Brian McNamara}
%\and
%\author{Tony Mroczkoski}
%\institute{European Southern Observatory (ESO), Karl-Schwarzschild-Strasse 2, Garching 85748, Germany}
%\institute{Max-Planck-Institut f\"{u}r Astrophysik (MPA), Karl-Schwarzschild-Strasse 1, Garching 85741, Germany}
%\and
%\author{Craig L. Sarazin}%r[0000-0003-0167-0981]
%\institute{Department of Astronomy, University of Virginia, 530 McCormick Road, Charlottesville, VA 22904-4325, USA}
%\and
%\author{Jonathon Sievers}
%\institute{ Department of Physics, McGill University, 3600 University Street Montreal, QC H3A 2T8, Canada}
%\and
%\author{Adrian Vantyghem}
%\and
%\author{Fernando Zago}
%\affiliation{Various}


